Learning to SHINE: Semiempirical Hamiltonians Informed by Machine-Learned Neighborhood Environments for Excited States

Despite advances in machine learning for molecular spectroscopy, predicting excitation energies and transition moments across unseen molecular scaffolds remains challenging. We introduce SHINE (Semiempirical Hamiltonians Informed by Machine-Learned Neighborhood Environments for Excited States), a machine learning model which uses frozen MACE representations and rotation-invariant descriptors of local chemical environments to learn bounded corrections to semiempirical Hamiltonians. Using the simplified Pariser--Parr--Pople (PPP) $\pi$-electron Hamiltonian, we train corrections through restricted Hartree--Fock and configuration interaction singles calculations and evaluate predictions against Tamm--Dancoff time dependent density functional theory references on molecular scaffolds excluded from training. Joint training on optical and spin targets improves excitation energies, the singlet--triplet gap, oscillator strengths, and transition moment magnitudes relative to fixed PPP. These gains hold in both the favorable population, drawn from the top 15% by reference $S_1$ local $\pi$ character, and the broader population without that cutoff. In the favorable population, the joint model reaches $S_1$, $T_1$ and signed gap mean absolute errors of 0.127, 0.118 and 0.105 eV, respectively. Within the same Hamiltonian, electric and magnetic transition moment magnitude errors are 0.270 $e\,a_0$ and 0.231 $\mu_{\mathrm{B}}$. Single-target supervision more than halves the joint model's $S_1$ and $T_1$ mean absolute errors, bringing them to 0.060 and 0.041 eV, respectively. The electric and magnetic specialists also lower their respective transition moment magnitude errors to 0.256 $e\,a_0$ and 0.224 $\mu_{\mathrm{B}}$. Together, these results show that learned corrections improve predictions within a reduced electronic description and motivate extending SHINE to richer semiempirical Hamiltonians.

==> desk24_main_references.tex <==
% Companion references exported from the current local build.
\newlabel{sec:introduction}{{1}{2}{Introduction}{section.1}{main.pdf}}
\newlabel{sec:methods}{{2}{6}{Methods}{section.2}{main.pdf}}
\newlabel{fig:1}{{1}{7}{Environmental features become a bounded Hamiltonian correction. The diagram follows one interacting pair along the \(\ell \) = 1 branch. Stacked cards represent four independent projection heads, each combining 224 encoder channels into eight query and eight key channels per angular order. Query--key~symmetric~contractions compare the environments, while pair-axis probes relate them to the connecting direction.~Across all the channels twelve environment-comparison scores, eight pair-axis probes, interatomic distance and the baseline interaction form the 22 inputs to the pair KAN.~Its scalar output passes through the bounded map to update the Hamiltonian parameter. The resulting core and Coulomb matrices enter PPP-RHF and singlet/triplet PPP-CIS to calculate the supervised properties. Gradients through these calculations train the projections and readouts while MACE remains frozen. Site readouts use 25 inputs, including four additional scalar features describing the individual environment and omitting the pair distance.~\relax }{figure.caption.1}{main.pdf}}
\newlabel{sec:ppp-hamiltonian}{{2.1}{8}{Environment-Dependent PPP Hamiltonian}{subsection.2.1}{main.pdf}}
\newlabel{sec:molecular-environment}{{2.1.1}{8}{Molecular Environment Features}{subsubsection.2.1.1}{main.pdf}}
\newlabel{sec:rotation-invariant-descriptors}{{2.1.2}{8}{Rotation-Invariant Descriptors}{subsubsection.2.1.2}{main.pdf}}
\newlabel{sec:kan-readouts}{{2.1.3}{9}{Kolmogorov--Arnold Network (KAN) Readouts}{subsubsection.2.1.3}{main.pdf}}
\newlabel{eq:source-03}{{1}{10}{Kolmogorov--Arnold Network (KAN) Readouts}{equation.2.1}{main.pdf}}
\newlabel{eq:source-04}{{2}{10}{Kolmogorov--Arnold Network (KAN) Readouts}{equation.2.2}{main.pdf}}
\newlabel{sec:bounded-corrections}{{2.1.4}{10}{Bounded Hamiltonian Corrections}{subsubsection.2.1.4}{main.pdf}}
\newlabel{eq:source-05}{{3}{11}{Bounded Hamiltonian Corrections}{equation.2.3}{main.pdf}}
\newlabel{eq:source-10}{{4}{11}{Bounded Hamiltonian Corrections}{equation.2.4}{main.pdf}}
\newlabel{sec:optical-spin-conventions}{{2.2}{11}{Optical Observables and Spin-Energy Conventions}{subsection.2.2}{main.pdf}}
\newlabel{fig:2}{{2}{12}{\textcolor {red}{Baseline parameters and learned corrections for the held-out molecule KAVHUL, evaluated with the favorable joint optical--spin model. Panels a--b show baseline on-site repulsions \(U_i^0\) and their learned changes; c--d show baseline core-diagonal elements \(h_{ii}^0\) and explicit site-energy offsets; e--f show baseline hoppings \(t_{ij}^0\) and their learned changes; g--h show the baseline intersite Coulomb matrix and its learned changes. The explicit site-energy offset is not the total change in the core diagonal. Grey bonds provide structural context outside the retained \(\pi \) space. Panel i compares carbon sites with the same baseline \(U\) (11.13 eV), with or without a non-\(\pi \) heavy-atom substituent: boxes show the interquartile range, the line the median and whiskers the 5th--95th percentiles.}\relax }{figure.caption.2}{main.pdf}}
\newlabel{eq:source-11}{{5}{13}{Optical Observables and Spin-Energy Conventions}{equation.2.5}{main.pdf}}
\newlabel{eq:source-12}{{6}{13}{Optical Observables and Spin-Energy Conventions}{equation.2.6}{main.pdf}}
\newlabel{eq:source-13}{{7}{13}{Optical Observables and Spin-Energy Conventions}{equation.2.7}{main.pdf}}
\newlabel{eq:source-14}{{8}{13}{Optical Observables and Spin-Energy Conventions}{equation.2.8}{main.pdf}}
\newlabel{eq:source-15}{{9}{13}{Optical Observables and Spin-Energy Conventions}{equation.2.9}{main.pdf}}
\newlabel{sec:formed-curation}{{2.3}{14}{FORMED Curation and Study Populations}{subsection.2.3}{main.pdf}}
\newlabel{sec:calculation-eligibility}{{2.3}{14}{FORMED Curation and Study Populations}{section*.3}{main.pdf}}
\newlabel{sec:reference-criteria}{{2.3}{14}{FORMED Curation and Study Populations}{section*.4}{main.pdf}}
\newlabel{sec:local-pi-character}{{2.3.1}{15}{\texorpdfstring {S\textsubscript {1} Local-\ensuremath {\pi } Character and the Favorable Population}{S1 Local-pi Character and the Favorable Population}}{subsubsection.2.3.1}{main.pdf}}
\newlabel{tab:1}{{1}{16}{Training, validation and test memberships of the two populations.\relax }{table.1}{main.pdf}}
\newlabel{sec:structural-descriptors}{{2.3}{16}{\texorpdfstring {S\textsubscript {1} Local-\ensuremath {\pi } Character and the Favorable Population}{S1 Local-pi Character and the Favorable Population}}{section*.5}{main.pdf}}
\newlabel{sec:scaffold-splits}{{2.3}{16}{\texorpdfstring {S\textsubscript {1} Local-\ensuremath {\pi } Character and the Favorable Population}{S1 Local-pi Character and the Favorable Population}}{section*.6}{main.pdf}}
\newlabel{sec:learning-objective}{{2.4}{17}{Learning Objective and Model Selection}{subsection.2.4}{main.pdf}}
\newlabel{eq:source-17}{{10}{17}{Learning Objective and Model Selection}{equation.2.10}{main.pdf}}
\newlabel{eq:source-18}{{11}{17}{Learning Objective and Model Selection}{equation.2.11}{main.pdf}}
\newlabel{sec:results}{{3}{19}{Results}{section.3}{main.pdf}}
\newlabel{sec:favorable-regime}{{3.1}{19}{Favorable Regime: \(\pi \)-Like S\textsubscript {1} Transitions}{subsection.3.1}{main.pdf}}
\newlabel{fig:3}{{3}{20}{Target-specific predictions of the five favorable specialists. Panels show \(\Delta E(\mathrm {S}_1)\), \(\Delta E(\mathrm {T}_1)\), \(f\) and \(\lVert \boldsymbol {\mu }\rVert \) and \(\lVert \mathbf {m}\rVert \) against their references. Teal filled points show SHINE-PPP specialist predictions and orange open circles show fixed PPP on the same molecules. Matching scalar-panel annotations give each method's MAE and Pearson r; n is the evaluation count. \textcolor {red}{Panel f compares electric and magnetic direction agreement: teal curves show the specialists and orange curves show fixed PPP on the same molecules; solid lines indicate \(\boldsymbol {\mu }\) and dashed lines indicate \(\mathbf {m}\).} The horizontal axis is the minimum absolute direction cosine with the reference, and the vertical axis is the fraction of molecules reaching that value. The table gives specialist and fixed-PPP median absolute cosines. Scalar panels use the common 884-molecule evaluation set; direction curves retain 884 electric and 771 magnetic comparisons after the resolution masks.\relax }{figure.caption.7}{main.pdf}}
\newlabel{fig:4}{{4}{21}{Favorable specialist accuracy transfers differently across properties. Rows show separately supervised models and columns show their supervised and unsupervised properties. Cells give MAE and its ratio to fixed PPP on the same molecules. All columns use the common 884-molecule favorable evaluation set, except \(\log _{10}|g_{\mathrm {abs}}|\) (694 molecules). Accepted finite zero or negative triplet predictions remain included.\relax }{figure.caption.8}{main.pdf}}
\newlabel{fig:6}{{5}{23}{Joint supervision balances target-specific accuracies in the favorable (a) and broad (b) populations. Errors are divided by fixed PPP's MAE on the same molecules: 1 denotes baseline accuracy, and values below 1 indicate improvement. \textcolor {red}{Each property uses separate horizontal lanes for fixed PPP, joint optical, joint optical--spin and specialist models. Colored numbers give MAE in the native units displayed with the property label at right; marker positions show the ratio to fixed PPP. Each specialist marker identifies the model trained on that property.} Comparisons use 884 favorable and 3,432 broad molecules, with 694 and 2,991, respectively, for \(\log _{10}|g_{\mathrm {abs}}|\). \textcolor {red}{Panel b omits relative-MAE values between 1.12 and 2.05 and compresses the scale to their right; paired slashes mark the break.}\relax }{figure.caption.9}{main.pdf}}
\newlabel{sec:broad-regime}{{3.2}{24}{Broad Regime: Bright, Resolved S\textsubscript {1} Transitions}{subsection.3.2}{main.pdf}}
\newlabel{fig:7}{{6}{25}{Target-specific predictions of the five broad specialists. Panels show \(\Delta E(\mathrm {S}_1)\), \(\Delta E(\mathrm {T}_1)\), \(f\) and \(\lVert \boldsymbol {\mu }\rVert \) and \(\lVert \mathbf {m}\rVert \) against their references. Teal filled points show specialist predictions and orange open circles show fixed PPP on the same molecules. Matching scalar-panel annotations give each method's MAE and Pearson r; n is the evaluation count. \textcolor {red}{Panel f compares electric and magnetic direction agreement: teal curves show the specialists and orange curves show fixed PPP on the same molecules; solid lines indicate \(\boldsymbol {\mu }\) and dashed lines indicate \(\mathbf {m}\).} The horizontal axis is the minimum absolute direction cosine with the reference, and the vertical axis is the fraction of molecules reaching that value. The table gives specialist and fixed-PPP median absolute cosines. Scalar panels use the common 3,432-molecule evaluation set; direction curves retain 3,432 electric and 3,151 magnetic comparisons after the resolution masks.\relax }{figure.caption.10}{main.pdf}}
\newlabel{fig:8}{{7}{26}{Broad specialist transfer depends on the supervised observable. Rows show the five specialists and columns their supervised and unsupervised properties. Cells give MAE and its ratio to paired fixed PPP. All columns use the common 3,432-molecule broad evaluation set, except \(\log _{10}|g_{\mathrm {abs}}|\) (2,991 molecules). Accepted finite zero or negative triplet predictions remain included.\relax }{figure.caption.11}{main.pdf}}
\newlabel{sec:discussion}{{4}{27}{Discussion}{section.4}{main.pdf}}
\newlabel{sec:learned-corrections}{{4.1}{27}{Environment Dependence of the Learned Corrections}{subsection.4.1}{main.pdf}}
\newlabel{fig:12}{{8}{28}{Molecular shift and within-molecule variation in the joint optical--spin model. The 880 favorable test molecules retained for the parameter analysis have at least four carbon sites and three C--C adjacent pairings. Each point summarizes carbon on-site repulsion or C--C hopping/intersite corrections: absolute molecular mean on the horizontal axis and population standard deviation on the vertical axis. The diagonal marks equality. Orange points identify KAVHUL. Its C--C hopping bars have mean +12.21\% and SD 4.69\%; the line and band show these quantities. C--C intersite corrections use 1.375 Å with raw learned outputs held fixed.\relax }{figure.caption.12}{main.pdf}}
\newlabel{tab:2}{{2}{28}{Molecular shift and within-molecule variation in the joint optical--spin model. Entries give separate medians over the 880 molecules. The final column divides median variation by the absolute median shift; it is not the median of per-molecule ratios. C--C intersite corrections are evaluated at 1.375 Å.\relax }{table.2}{main.pdf}}
\newlabel{sec:limitations}{{4.2}{29}{Limitations and Outlook}{subsection.4.2}{main.pdf}}
\newlabel{sec:reduced-orbital-basis}{{4.2}{29}{Limitations and Outlook}{section*.13}{main.pdf}}
\newlabel{sec:singles-only-treatment}{{4.2}{29}{Limitations and Outlook}{section*.14}{main.pdf}}
\newlabel{sec:conclusion}{{5}{30}{Conclusion}{section.5}{main.pdf}}

